3D Phase Retrieval at Nano-Scale via Accelerated Wirtinger Flow

Imaging 3D nano-structures at very high resolution is crucial in a variety of scientific fields. However, due to fundamental limitations of light propagation we can only measure the object indirectly via 2D intensity measurements of the 3D specimen through highly nonlinear projection mappings where a variety of information (including phase) is lost. Reconstruction therefore involves inverting highly non-linear and seemingly non-invertible mappings. In this paper, we introduce a novel technique where the 3D object is directly reconstructed from an accurate non-linear propagation model. Furthermore, we characterize the ambiguities of this model and leverage a priori knowledge to mitigate their effect and also significantly reduce the required number of measurements and hence the acquisition time. We demonstrate the performance of our algorithm via numerical experiments aimed at nano-scale reconstruction of 3D integrated circuits. Moreover, we provide rigorous theoretical guarantees for convergence to stationarity.

==> ambiguity.tex <==
\section{Ambiguity challenge}\label{sec:ambi}
Recovering the phase of the ground truth object based on phaseless measurements is only possible up to a certain factor of ambiguity due to phase wrapping effects originating in the projection model in Eq. \ref{eq:gl}. When we discuss the Radon-transform of the object in a certain orientation, that is $\vct{p}_l = \mtx{T}_l \vct{x}$, we refer to it as the projection image in orientation $l$. When we talk about $\gl$, which we obtain from scaling and exponentiating the projection image, we refer to it as the exit wave in orientation $l$.  In this section, we aim at formalizing this ambiguity and offering means to counter its effect on the final reconstruction. 

Let $\vct{x}^* = \vct{d}^* + i \vct{b}^*$ be the ground truth object we wish to reconstruct and  $\hat{\vct{x}} = \hat{\vct{d}} + i \hat{\vct{b}}$ be the estimated object obtained from our reconstruction algorithm. Furthermore, we write  $\hat{\vct{d}} = \vct{d}^* + \tilde{\vct{d}}$, where $\tilde{\vct{d}}$ is the error in the real part of the reconstruction. Then the reconstructed exit wave in orientation $l$ takes the form
%\begin{align}
%\hat{\gl} &=  exp(i \frac{2\pi}{\lambda}\mtx{T}_l \hat{x})= exp(i \frac{2\pi}{\lambda}\mtx{T}_l (\vct{d}^* + \tilde{\vct{d}} + \hat{\vct{b}} i)) \nonumber\\
% &= exp(-\frac{2\pi}{\lambda}\hat{\vct{b}}) \cdot exp(i\frac{2\pi}{\lambda}\mtx{T}_l \vct{d}^*) \cdot exp(i\frac{2\pi}{\lambda}\mtx{T}_l \tilde{\vct{d}}).
%\end{align}
\begin{align}
\hat{\gl} &= e^{-\frac{2\pi}{\lambda}\hat{\vct{b}}} \cdot e^{i\frac{2\pi}{\lambda}\mtx{T}_l \vct{d}^*} \cdot e^{i\frac{2\pi}{\lambda}\mtx{T}_l \tilde{\vct{d}}}.
\end{align}

Taking a look at the right hand side we may conclude that: (1) the imaginary part of the refractive index has no effect on the phase and does not cause ambiguity in the exit wave, and (2) if we let $\mtx{T}_l \tilde{\vct{d}} = \lambda \vct{K}$ for any $\vct{K} \in \mathbb{Z}^{P}$ will be consistent with the measurements and our model is not able to differentiate between the reconstruction and the ground truth exit wave.
%
%To elaborate further, consider an incident beam $B^l_j$ at angle $l$ that produces pixel $\hat{p}^l_j$ on the projection image (its real part to be more specific). Denote $I:\{i| x_i \in B^l_j\}$ the set of indices of voxels intersected by the beam. Explicitly writing out the Radon-transform for this pixel is simply a sum in the discrete case:
%$\hat{p}^m_j =  \sum_{i \in I} \hat{\vct{d}}_i=  \sum_{i \in I} d_i^* +\sum_{i \in I} \tilde{d}_i. $
%Assume that the voxel-wise reconstruction error can be written as 
%$\tilde{d}_i = k_i \lambda, ~k_i \in \mathbb{Z} ~ \forall i,$
%and in this case
%$$\hat{p}^m_j =  \sum_{i \in B} d_i^* +\lambda \sum_{i \in B} k_i =\sum_{i \in B} d_i^* +\lambda k',$$
%which results in the same exit wave pixel as the ground truth object and therefore indistinguishable from the ground truth in our model. Moreover, due to phase wrapping we lose all information on individual $k_i$'s (even $\sum_{i \in B} k_i $ which is known in the projection image, but not after exponentiation).  In other words, adding some $ \lambda k", ~k" \in \mathbb{Z}$ to any $\hat{d}_i$ will not change the cost function nor any of the exit waves. 

%This ambiguity is different from the case when we take $A T_m x$ as our propagation model (without exponentiation), because in that case we retain the information on $\sum_{i \in B} k_i $ and therefeore $k_i$'s are connected between different angles.

